Chirality Effects in Molecular Chainmail

Motivated by the observation of positive Gaussian curvature in kinetoplast DNA networks, we consider the effect of linking chirality in square lattice molecular chainmail networks using Langevin dynamics simulations and constrained gradient optimization. Linking chirality here refers to ordering of over-under versus under-over linkages between a loop and its neighbors. We consider fully alternating linking, maximally non-alternating, and partially non-alternating linking chiralities. We find that in simulations of polymer chainmail networks, the linking chirality dictates the sign of the Gaussian curvature of the final state of the chainmail membranes. Alternating networks have positive Gaussian curvature, similar to what is observed in kinetoplast DNA networks. Maximally non-alternating networks form isotropic membranes with negative Gaussian curvature. Partially non-alternating networks form flat diamond-shaped sheets which undergo a thermal folding transition when sufficiently large, similar to the crumpling transition in tethered membranes. We further investigate this topology-curvature relationship on geometric grounds by considering the tightest possible configurations and the constraints that must be satisfied to achieve them.

==> extratext.tex <==
%the aforementioned Hopf link and add a third loop that is Hopf linked to both previous loops, forming a chain, and then link both ends of the chain together forming a triangle. The connection may be made such that all crossings alternate over-under, forming the $6_{3}^{1}$ link. Each loop is rotationally constrained in this configuration. If instead the ends are connected such that the crossings may be described as over FINISH THIS.

%This chiralilty may be extended to larger networks and lattices of links. A unit cell may be defined such that each loop has a sequence of over-under relations with its neighbors, which can then tile a plane. In this case, the choice of chirality may have large-scale effects on the network's geometric configuration. This was explored by He et al. for honeycomb lattices, which are superpositions of two triangular lattices. Each loop in one triangular lattice is connected to three loops in the other triangular lattice, each of which it may go over-under or under-over, leading to 8 different possible configurations for each loop. Although it was noticed that the choice of chirality may affect the curvature of a molecule, a choice was made to neutralize this effect by randomizing the chirality of each locus. The earlier work by Polson, Garcia, and Klotz simulated Japanese-style chainmail in which loops in a lattice with valence 4 were each connected by non-lattice loops with valence 2. This configuration lacked a chiral constraint. In a preliminary set of simulations exploring effects of various molecular chainmail topologies, chiral effects were also noticed by Thomas O'Connor.

%Here, we consider the effect of molecular chirality in square lattices of topologically linked loops. Although the honeycomb lattice is typically used to describe kinetoplast DNA, we choose the square lattice because the chirality can be varied in the unit cell without inducing frustration. Additionally, the 4-valence yields a bigger difference between the fully alternating and fully non-alternating cases. Consider a loop that is Hopf linked to four of its neighbors, each of which cannot be rotated (for simplicity, place one at each cardinal compass direction). Going around the loop and describing whether it passes over or under each neighbor, there are a total of eight crossings, four of which are over and four of which are under. The fully alternating configuration is over-under-over-under-over-under-over-under. If two opposite neighbors are flipped (say North and South), the crossings may be read as over-over-under-under-over-over-under-under, which is the maximally non-alternating configuration. If two adjacent neighbors are flipped (say North and East), the crossings may be read as over-over-under-over-under-under-over-under, the partially non-alternating configuration.

%Here, we consider the effect of this chirality in the configurations of molecular chainmail network. We consider two types of configuration: the ``ideal'' configuration which minimizes the total contour length of the network while satisfying a no-overlap constraint on the loops, and the thermal equilibrium configuration that is reached when each loop is treated as a polymer chain similar to a kinetoplast minicircle. The former allows us to explore the effect of these chiral constraints from a purely geometric standpoint, while the latter allows us to investigate what role chirality may play in determining the structure of kinetoplast networks.

%Consider the three 8-crossing, 4-element links: $8_{4}^1$, $8_{4}^2$, and $8_{4}^3$ or L8a21, L8n7, and L8n8. These can be thought of as four-loop closed chains, in which each loop is linked to two others. The first is fully alternating, each loop reads as a sequence of over-unders. When tightened it has a ropelength of at most 75.3. The second is partially alternating, with two links reading as over-under-over-under and two reading as over-over-under-under. It has a roplength of at most 67.4. The third has all four loops reading as over-over-under-under, and has a ropelength of at most 66.3. In this case, we can compute the ropelength exactly, as it is made of four stadium curves each with contour length $4\pi+4$, giving it a total ropelength of $16\pi+16\approx 66.27$, within 0.1\% of the computed value. The alternating links cannot form perfect stadia as the have to twist to accomodate their neigbhors.

